Between burning and cooling: liminal burning on graphs

Liminal burning generalizes both the burning and cooling processes in graphs. In $k$-liminal burning, a Saboteur reveals $k$-sets of vertices in each round, with the goal of extending the length of the game, and the Arsonist must choose sources only within these sets, with the goal of ending the game as soon as possible. The result is a two-player game with the corresponding optimization parameter called the $k$-liminal burning number. For $k = |V(G)|$, liminal burning is identical to burning, and for $k = 1$, liminal burning is identical to cooling. Using a variant of Sperner sets, $k$-liminal burning numbers of hypercubes are studied along with bounds and exact values for various values of $k$. In particular, we determine the exact cooling number of the $n$-dimensional hypercube to be $n.$ We analyze liminal burning for several graph families, such as Cartesian grids and products, paths, and graphs whose vertex sets can be decomposed into many components of small diameter. We consider the complexity of liminal burning and show that liminal burning a graph is PSPACE-complete for $k\geq 2,$ using a reduction from $3$-QBF. We also prove, through a reduction from burning, that even in some cases when liminal burning is likely not PSPACE-complete, it is co-NP-hard. We finish with several open problems.

==> Th11_LBhypercubes.tex <==

%
We also have the following lower bound. 
%
\begin{theorem}\label{thm:down1}
Let $k,n$ be integers. 
Suppose $d$ is such that $\sum_{i=0}^{d-2}\binom{n}{i}\geq k$ and
%
\begin{equation}\label{eq:bigendian}
\binom{\big\lceil\frac{n+2}{2}\big\rceil +d}{d} \geq \left(\Big\lfloor\frac{n-2}{2}\Big\rfloor -d+1\right)\cdot k.
\end{equation}
%
It follows that 
%
\begin{equation*}
    b_k(Q_n) \geq \begin{cases}
        n -2d+1 & \text{if }n\text{ is odd,} \\
        n-2d+2 & \text{if }n\text{ is even.}
    \end{cases}
\end{equation*}
\end{theorem}

Unpacking all the values of $d$ and $k$ when the hypotheses of Theorem~\ref{thm:down1} apply appears challenging given the asymptotics of sums of binomial coefficients. Nevertheless, for sufficiently large $n$, $k = o(n^{d-2})$ satisfies both conditions imposed by Theorem~\ref{thm:down1}. Therefore, for such $k$ we have that $b_{k}(Q_n) \geq n-2d+1$ for large enough $n$. In particular, for $d = 3$ and $k \leq n+1$, we derive that $b_k(Q_n) \ge n-5$. 

\begin{proof}[Proof of Theorem~\ref{thm:down1}]
We provide a Saboteur strategy that lasts $n-2d-1$ rounds when $n$ is odd and $n-2d$ rounds otherwise. 
Let \textit{level} $i$ be the set of all vertices of distance $i$ from the vertex $\emptyset$.
We begin by showing that the Saboteur can play $\lfloor\frac{n-2}{2}\rfloor -d+2$ rounds such that no vertex in level greater than $\lfloor\frac{n-2}{2}\rfloor$ is burned. 

We enforce the following rules, which only benefit the Arsonist, to simplify analysis:
For all rounds, we burn all revealed vertices during the Arsonist's move; 
the Saboteur plays the first round by revealing the $\sum_{i=0}^{d-2}\binom{n}{i}\geq k$ vertices that are closest to the vertex $\emptyset$, which are only vertices of level $d-2$ or lesser; 
finally, all vertices of level $d-2$ or lesser are burned during the first round. 
Thus, at the start of the second round, all vertices in level $d-1$ are burned by propagation.

Consider the ordering on the vertices of each level where vertex $u$ is lesser than vertex $v$ if there exists $m \in v \setminus u$ such that $m$ is strictly less than each element of $u \setminus v$. 
If level $d+i-2$ always contains at least $k$ unburned vertices at the start of the Saboteur's $i$th move with $2 \leq i \leq \lfloor \frac{n-2}{2}\rfloor -d+2$, then vertices of level at most $d+i-3$ are burned, vertices of level $d+i-2$ may be burned or unburned, and vertices of level $d+i-1$ or more are unburned. 
After propagation in round $i+1$, vertices of level at most $d+i-2$ are burned, vertices of level $d+i-1$ may be burned or unburned vertices, and vertices of level $d+i$ or more are unburned. 
Let $\overline{v}_i$ be the greatest vertex in level $d+i-2$ burned by the $i$-th propagation step and let $v_i$ be the greatest vertex in level $d+i-2$ burned by the Arsonist's $i$-th move. 

Let $S$ denote the set of subsets of $\{ \lfloor\frac{n-2}{2}\rfloor-d+1, \ldots, n\}$ that have cardinality $d$, noting that $\{ \lfloor\frac{n-2}{2}\rfloor-d+1, \ldots, n\}$ is the set of the last $\lceil \frac{n+2}{2} \rceil +d$ elements in $[n]$. 
We define two subsets $\overline{w}_i$ and $w_i$ such that both $w_i$ and $\overline{w}_i$ contain the first $i-2$ elements of $[n]$, such that both do \textit{not} contain the next $\lfloor\frac{n-2}{2}\rfloor-d-i+2$ elements of $[n]$. 
Further, $\overline{w}_i$ contains each element in the $((i-2)k)$-th smallest subset that is an element of $S$ and $w_i$ contains the elements of the $((i-1)k)$-th smallest subset that is an element of $S$.
We consider $w_i$ to be defined for $i>2$ and $\overline{w}_i$ to be defined for $i \geq 2$. 
We will show inductively that $w_i \geq v_i$ and $\overline{w}_{i+1} \geq \overline{v}_{i+1},$ beginning with the former.

We assume for induction that $\overline{w}_i \geq \overline{v}_i$. 
{\color{red}Trent: (BASES CASE HERE. Might be a little convoluted)}
During the Saboteur's $i$-th move, they reveal the $k$ smallest unburned vertices in level $d+i-2$.
Since no burned vertex on this level is larger than $\overline{w}_i$, there are $k$ unburned vertices on this level that correspond to changing the last $\lceil \frac{n-2}{2} \rceil +d$ elements of $\overline{w}_i$ to be the $[(i-2)k+1]$-th smallest subset through to the $(i-1)k$-th smallest subset of $S$. 
By \eqref{eq:bigendian}, there are always enough such subsets.
The largest of this set of $k$ unburned vertices is $w_i$, so the largest revealed vertex is less than $w_i$, and so all vertices burned during the Arsonist's move, including $v_i$, are less than or equal to $w_i$, completing the first part of the induction. 

We now show that $\overline{w}_{i+1} \geq \overline{v}_{i+1}$.  
By definition, $\overline{v}_{i+1}$ is the greatest vertex of level $d+i-1$ burned in the $(i+1)$-th propagation step. 
Also, $\overline{v}_{i+1}$ is exactly the subset $v_{i}$, except that it contains the smallest element of $[n]\setminus v_{i}$. 
{\color{red} Trent: Stopped here for now. We will need to compare $\overline{v}_{i+1}$ to $\overline{w}_{i+1}$, and we can claim that if the former is biger by our ordering, then we get a contradiction. Also note the following line is incorrect in general. }
Therefore, $\overline{v}_i=\overline{w}_{i}$, completing the induction. 

We have so far played the first $\lfloor \frac{n-2}{2} \rfloor-d+2$ rounds such that no vertices in level $d+\lfloor \frac{n-2}{2} \rfloor-d+2 = \lfloor \frac{n}{2}\rfloor$ are burned, and now show that a further $\lfloor \frac{n-2}{2} \rfloor-d+2$ rounds can be played. 
To simplify analysis, we assume that all vertices in level $\lceil \frac{n}{2}\rceil -1$ or before are burned, noting that this burns an extra level when $n$ is odd.
Let $S_i$ be the set of $k$ vertices that were revealed in round $i$ for $1 \leq i \leq \lfloor \frac{n-2}{2} \rfloor-d+2$, and note that $S_i$ must have distance at least $e+1$ from $S_{i+e}$ for any $e$, or else the vertices in $S_{i+e}$ would have been burned before they were revealed. 

For a set $A$, let $A^c$ be its complement. Define $S'_{i} = \{A^c: A\in S_{2\lfloor\frac{n-2}{2}\rfloor -2d +5 - i}\}$ for $\lfloor \frac{n-2}{2}\rfloor -d+3 \leq i \leq 2\lfloor \frac{n-2}{2} \rfloor -2d+4$. The set $S'_i$ has distance at least $e+1$ from $S'_{i-e}$, since $|A\Delta B| = |A^c \Delta B^c|$. Also, the subsets in $S'_i$ contain $i+d-1$ elements and are in level $i+d-1$.

Suppose for induction that in round $\lfloor \frac{n-2}{2}\rfloor -d+3 \leq i \leq 2\lfloor \frac{n-2}{2} \rfloor -2d+4$, the set $S'_i$ is unrevealed. This is true in the base case when $i=\lfloor \frac{n-2}{2}\rfloor -d+3.$
Now suppose that the Saboteur reveals $S'_i$ during round $i$ and that $S'_i$ is burned during the Arsonist's move in this round. 
After propagation in round $i+1$, the vertices in level $i+d-1$ or before are burned, the vertices in level $i + d +1$ or after are not burned, and the vertices in level $i+d$ are burned if and only if they are distance $e$ to $S'_{i+1-e}$ for some $e\geq 1$.
Since $S'_{i+1}$ is distance $e+1$ to $S'_{i+1-e}$, the vertices in $S'_{i+1}$ are not burned, and may be revealed by the Saboteur during the next round, completing the induction. Thus, the game lasts for at least $2\lfloor \frac{n-2}{2} \rfloor -2d+4$ rounds.
\end{proof}

Combining Theorem~\ref{thm:up1} and Theorem~\ref{thm:down1}, we have the following corollary.

\begin{corollary}
    Let $c$ be a positive integer greater than $1$ and $k = \Theta(n^c)$. For sufficiently large $n$, $$n - 2c - 5 \leq b_k(Q_n) \leq n-c + 2.$$ 
\end{corollary}

\begin{proof}
    Since $k = \Theta(n^c)$ we have $k = \omega(n^{c-1})$ and $k = o(n^{c+1})$. The discussion following the statement of Theorem~\ref{thm:down1} gives the lower bound by taking $d - 2 = c + 1$. For the upper bound, observe that $k = \omega(n^{c-1})$ implies $k = \omega(n)$ and $k = \Theta(n^c)$ implies $k = o(2^n)$ and so for sufficiently large $n$ the conditions of Theorem~\ref{thm:up1} are satisfied by $d = c - 1$.
\end{proof}

==> unused.tex <==
\begin{theorem}\label{thm:down1}
Let $k,n$ be integers. 
Suppose $d$ is such that $\sum_{i=0}^{d-2}\binom{n}{i}\geq k$ and
\[
\binom{\big\lceil\frac{n+2}{2}\big\rceil +d}{d} \geq \left(\Big\lfloor\frac{n-2}{2}\Big\rfloor -d+1\right)\cdot k.\]
It follows that when $n$ is odd,
\[b_k(Q_n)\geq n-2d+1,\] 
and when $n$ is even
\[b_k(Q_n)\geq n-2d+2.\] 
\end{theorem}

One of the consequences of Theorem~\ref{thm:down1} is that $b_n(Q_n) \ge n-5$ (where we choose $d=3$ and $k=n).$ Unpacking all the values of $d$ and $k$ when the hypotheses of Theorem~\ref{thm:down1} apply appears challenging given the asymptotics of binomial coefficients.

\begin{proof}[Proof of Theorem~\ref{thm:down1}]
We provide a Saboteur strategy that takes at least 
$n-2d-1$
rounds in the case that $n$ is odd, and 
$n-2d$
rounds in the case that $n$ is even. 
To begin, we will show that the Saboteur can play 
$\lfloor\frac{n-2}{2}\rfloor -d+2$ 
rounds while ensuring that no vertex of distance greater than $\lfloor\frac{n-2}{2}\rfloor$ from the vertex $\overline{0}$ is burned. 
We define level $i$ to be the set of all vertices of distance $i$ from the vertex $\overline{0}$. 

For all rounds, we may disadvantage the Saboteur by burning all vertices during the Arsonist's move, making the Arsonist's strategy redundant. 
The Saboteur plays their first round by selecting the $k$ vertices that are closest to the vertex $\overline{0}$, with ties broken arbitrarily.
Since $\sum_{i=0}^{d-2}\binom{n}{i}\geq k$, only vertices on level $d-2$ or before are revealed and subsequently burned by the Arsonist. 
Disadvantaging the Saboteur further, we may burn all vertices of level $d-2$ or before at the end of the first round. 
At the start of the second round, the propagation step burns all vertices on level $d-1$.

We identify the vertices of $Q_n$ with \emph{binary words}, which are binary strings of length $n.$
Consider the ordering on the vertices of each level such that a vertex $u$ comes earlier in the ordering than vertex $v$ if the binary word corresponding to $u$ is smaller than the binary word corresponding to $v$. 
If level $d+i-2$ always contains at least $k$ unburned vertices at the start of the Saboteurs $i$th move with $2 \leq i \leq \lfloor \frac{n-2}{2}\rfloor -d+2$, then it is straightforward to see that all vertices of level at most $d+i-3$ have previously been burned, the vertices of level $d+i-2$ may contain both burned and unburned vertices, and the vertices of level $d+i-1$ or more have not been burned. 
Let $v_i$ be the newly-burned vertex of level $d+i-2$ after the Arsonist's move in round $i$ that comes latest in the ordering. 
After the propagation of round $i+1$, all vertices of level at most $d+i-2$ have been burned, the vertices of level $d+i-1$ may contain both burned and unburned vertices, and the vertices of level $d+i$ or more have not been burned. 
Let $\overline{v}_i$ be the newly-burned vertex of level $d+i-1$ after the propagation of round $i$ that comes latest in the ordering. 

 We consider the binary words to be \emph{big-endian} in the sense that when we compare two binary words, the first digit is the most significant bit in determining which is larger.  We define two words of length $n$, $w_i$ and $\overline{w}_i$. 
Define the first $i-2$ digits of both $\overline{w}_i$ and $w_i$ be ones and the next $(\lfloor\frac{n-2}{2}\rfloor-d+2)-(i-2)$ digits be zeroes. 
Define the last $\lceil \frac{n-2}{2} \rceil +d$ digits of $w_i$ and $\overline{w}_{i+1}$ be the $((i-2)k)$th smallest word of length $\lceil \frac{n-2}{2} \rceil +d$ containing $d$ ones. 
We will show inductively that $w_i$ is larger than or equal to the binary word corresponding to $v_i$ and that $\overline{w}_i$ is larger than or equal to the binary word corresponding to $\overline{v}_i$.

We begin by showing that the binary word corresponding to $v_i$ is less than or equal to $w_i$. 
During the Saboteurs' $i$th move, the Saboteur reveals the $k$ smallest vertices from the set of unburned vertices of level $d-i+2$ according to the ordering. 
The last $\lceil \frac{n-2}{2} \rceil +d$ digits of $\overline{w}_i$ form the $((i-2)k)$th smallest word from the set of words of length $\lceil \frac{n-2}{2} \rceil +d$ that contains $d$ words. 
Since no burned vertex on this level has corresponding binary word larger than $\overline{w}_i$, there are $k$ unburned vertices on this level that correspond to changing the last digits of $\overline{w}_i$ to be the $((i-2)k+1)$th smallest word through to the $((i-1)k)$th smallest word. 
This is valid, since by our assumption $\binom{\lceil\frac{n+2}{2}\rceil +d}{d} \geq \left(\lfloor\frac{n-2}{2}\rfloor -d+1\right)\cdot k,$ and so there are enough such words.
Label the largest of this set of $k$ unburned vertices as $v$, which has the corresponding binary word $w_i$. 
Hence, the largest revealed vertex occurs earlier in the ordering than $v$, and so all vertices burned during the Arsonist's move have corresponding word at most $w_i$. 
We further disadvantage the Saboteur by burning all vertices on this level that have a corresponding word of $w_i$ or less. 
This completes the first part of the induction. 

We complete the induction by showing that the binary word corresponding to $\overline{v}_{i+1}$ is less than or equal to $\overline{w}_{i+1}$. 
During the propagation step of round $i+1$, exactly the vertices of distance $1$ from the previously burned vertices are then burned. 
Let $\overline{v}_{i+1}$ be the burned vertex of level $d+i-1$ that comes latest in the ordering, with corresponding binary word $w$. 
Note that $w$ is exactly the word $w_i$ but with its $(i-1)$th digit, which was previously a $0$, exchanged for a $1$. 
Therefore, $w=\overline{w}_{i+1}$, and the induction is complete. 

After round $\lfloor \frac{n-2}{2} \rfloor-d+2$, we then have that no vertices on level  $d+\lfloor \frac{n-2}{2} \rfloor-d+2 = \lfloor \frac{n}{2}\rfloor$ have been burned. 
Further disadvantaging the Saboteur, we assume at this point that all vertices on level $\lceil \frac{n}{2}\rceil -1$ or before are burned, noting that in the case that $n$ is odd, one additional full level has been burned compared with the even case. 

We have so far played the first $\lfloor \frac{n-2}{2} \rfloor-d+2$ rounds, and we will proceed to show that a further $\lfloor \frac{n-2}{2} \rfloor-d+2$ rounds can be played. 
Let $S_i$ be the set of $k$ vertices that were played in round $i$ for $1 \leq i \leq \lfloor \frac{n-2}{2} \rfloor-d+2$. 
Note that the words in $S_i$ have distance at least $e+1$ to the words in $S_{i+e}$, or else the vertices corresponding to the words in $S_{i+e}$ would have been burned before they were revealed. 

The \emph{binary inversion} of a word is the word resulting from interchanging the 0's and 1's in the original word. 
Define $S'_{i}$ to be the set of words formed by taking the binary inversion of the words in $S_{2\lfloor\frac{n-2}{2}\rfloor -2d +5 - i}$ for $\lfloor \frac{n-2}{2}\rfloor -d+3 \leq i \leq 2\lfloor \frac{n-2}{2} \rfloor -2d+4$. 
We note that each word in $S'_i$ has distance at least $e+1$ to the words in $S'_{i-e}$, since word inversion on two words does not change the distance between them. 
Note that the words in $S'_i$ each have $i+d-1$ ones, and so the corresponding vertices are on level $i+d-1$. 

Suppose for induction that in round $i$, the set of $k$ vertices with corresponding words $S'_i$ have not been revealed, with $\lfloor \frac{n-2}{2}\rfloor -d+3 \leq i \leq 2\lfloor \frac{n-2}{2} \rfloor -2d+4$. 
This is true for the base case when $i=\lfloor \frac{n-2}{2}\rfloor -d+3$
The Saboteur reveals this set of $k$ vertices of round $i$. 
These $k$ vertices are then burned during the Arsonist's move in this round. 
After the propagation of round $i+1$, the vertices on level $i+d-1$ or before are all burned, the vertices on level $i + d +1$ or after are not burned, and the vertices of level $i+d$ are burned if and only if they have distance $e$ to a word in $S'_{i+1-e}$ for some $e\geq 1$.
Since the vertices in $S'_{i+1}$ have distance $e+1$ to any word in $S'_{i+1-e}$, the vertices in $S'_{i+1}$ have not been burned, and so may be revealed by the Saboteur during the next round, completing the induction. 

We have thus shown that the Saboteur can make the game last for at least $2\lfloor \frac{n-2}{2} \rfloor -2d+4$ rounds.  
The result follows when we split into the odd and even cases. 
\end{proof}
